Locality-aware Cross-modal Correspondence Learning for Dense Audio-Visual Events Localization

Dense-localization Audio-Visual Events (DAVE) aims to identify time boundaries and corresponding categories for events that are both audible and visible in a long video, where events may co-occur and exhibit varying durations. However, complex audio-visual scenes often involve asynchronization between modalities, making accurate localization challenging. Existing DAVE solutions extract audio and visual features through unimodal encoders, and fuse them via dense cross-modal interaction. However, independent unimodal encoding struggles to emphasize shared semantics between modalities without cross-modal guidance, while dense cross-modal attention may over-attend to semantically unrelated audio-visual features. To address these problems, we present LoCo, a Locality-aware cross-modal Correspondence learning framework for DAVE. LoCo leverages the local temporal continuity of audio-visual events as important guidance to filter irrelevant cross-modal signals and enhance cross-modal alignment throughout both unimodal and cross-modal encoding stages. i) Specifically, LoCo applies Local Correspondence Feature (LCF) Modulation to enforce unimodal encoders to focus on modality-shared semantics by modulating agreement between audio and visual features based on local cross-modal coherence. ii) To better aggregate cross-modal relevant features, we further customize Local Adaptive Cross-modal (LAC) Interaction, which dynamically adjusts attention regions in a data-driven manner. This adaptive mechanism focuses attention on local event boundaries and accommodates varying event durations. By incorporating LCF and LAC, LoCo provides solid performance gains and outperforms existing DAVE methods.

==> tabs/ab_study.tex <==
\begin{table*}[t!]
        \centering
	\begin{subtable}
  {0.5\linewidth}
  \resizebox{0.98\textwidth}{!}{
			\setlength\tabcolsep{4.4pt}			\renewcommand\arraystretch{1.0}
    \begin{tabular}{cc|cccccc}
\thickhline
\rowcolor{mygray}  LCC & CDP & 0.5 & 0.6 & 0.7 & 0.8 & 0.9 & Avg. \\

\hline
\hline

&  & $37.1$ & $29.0$ & $21.6$ & $13.6$ & $6.9$ & $37.0$ \\
\cmark & & $45.6$ & $38.8$ & $32.0$ & $25.2$ & $17.3$ & $45.2$ \\
 & \cmark & $56.0$ & $51.1$ & $43.6$ & $35.6$ & $23.0$ & $52.5$ \\
\textbf{{\cmark}} & \textbf{{\cmark}} & $\mathbf{56.6}$ & $\mathbf{51.4}$ & $\mathbf{44.7}$ & $\mathbf{36.7}$ & $\mathbf{25.9}$ & $\mathbf{53.4}$ \\

\hline
\end{tabular}
	}
		
		\setlength{\abovecaptionskip}{0.18cm}
		\setlength{\belowcaptionskip}{0.12cm}
		\caption{Key Component Analysis}
		
        \label{ab1}
	\end{subtable}
        \hspace{-1.0em}     
        \begin{subtable}{0.5\linewidth}
         \centering
           
		\resizebox{0.98\textwidth}{!}{
			\setlength\tabcolsep{2.5pt}
			\renewcommand\arraystretch{0.95}
        \begin{tabular}{c|cccccc}
\thickhline
\rowcolor{mygray}  $\bm{G}$-type & 0.5 & 0.6 & 0.7 & 0.8 & 0.9 & Avg. \\
\hline
\hline
Diagonal matrix & $55.9$ & $51.1$ &$44.1$ &$35.4$ &$21.9$ &$52.7$ \\
Softened target & $55.6$  & $50.5$ & $43.9$ & $36.6$& $23.1$&$52.8$ \\
Fixed gaussian  & $55.9$ &$50.9$ &$44.4$ &$\mathbf{36.8}$ &$23.7$ &$52.9$ \\ 
\textbf{Ours} & $\mathbf{56.6}$ & $\mathbf{51.4}$ & $\mathbf{44.7}$ & $36.7$ & $\mathbf{25.9}$ & $\mathbf{53.4}$ \\
\hline
\end{tabular}
}
		
		\setlength{\abovecaptionskip}{0.15cm}
		\setlength{\belowcaptionskip}{0.15cm}
		\caption{Types of Correspondence Objective $\bm{G}$}
		\label{ab2}
	\end{subtable} \\
	\begin{subtable}{0.5\linewidth}
  \centering
		\resizebox{0.98\textwidth}{!}{
			\setlength\tabcolsep{2.5pt}
	\renewcommand\arraystretch{1.33}
       \begin{tabular}{c|cccccc}
\thickhline
\rowcolor{mygray}  Attention strategy & 0.5 & 0.6 & 0.7 & 0.8 & 0.9 & Avg. \\

\hline
\hline
 
Global & $55.5$ & $50.2$ & $43.9$ & $36.4$ & $22.6$ & $52.4$ \\
Fixed  & $56.4$ & $50.6$ & $43.9$ & $35.3$ & $22.5$ & $52.7$ \\
\textbf{CDP} & $\mathbf{56.6}$ & $\mathbf{51.4}$ & $\mathbf{44.7}$ & $\mathbf{36.7}$ & $\mathbf{25.9}$ & $\mathbf{53.4}$ \\

\hline
\end{tabular}	}
		
		\setlength{\abovecaptionskip}{0.2cm}
		\setlength{\belowcaptionskip}{-0.1cm}
		\caption{Cross-modal Dynamic Perception}
		\label{ab3}
	\end{subtable}
        \hspace{-0.7em}
	\begin{subtable}{0.5\linewidth}
  \centering
        \small
		\resizebox{0.98\textwidth}{!}{
			\setlength\tabcolsep{2.5pt}
			\renewcommand\arraystretch{0.9}
  \begin{tabular}{c|cccccc}
\thickhline
\rowcolor{mygray}  Base window size & 0.5 & 0.6 & 0.7 & 0.8 & 0.9 & Avg. \\

\hline
\hline
 
$4$ & $55.8$ & $50.6$ & $44.3$ & $36.5$ & $25.4$ & $52.9$ \\
$\mathbf{8}$  & $\mathbf{56.6}$ & $\mathbf{51.4}$ & $44.7$ & $\mathbf{36.7}$ & $\mathbf{25.9}$ & $\mathbf{53.4}$ \\
$16$ & $56.2$ & $51.3$ & $\mathbf{44.9}$ & $36.6$ & $25.1$ & $53.0$ \\
$32$ & $56.2$ & $51.3$ & $44.2$ & $36.0$ & $23.2$ & $52.8$ \\
Full & $55.5$ & $50.2$ & $43.9$ & $36.4$ & $22.6$ & $52.4$ \\
\hline
\end{tabular}
		}	
		\setlength{\abovecaptionskip}{0.2cm}
		\setlength{\belowcaptionskip}{-0.1cm}
		\caption{Base Window Size}
		\label{ab4}
	\end{subtable}
\makeatletter\def\@captype{table}\makeatother\captionsetup{font=small}\caption{\small $_{\!}$A$_{\!}$ set$_{\!}$ of$_{\!}$ \textbf{ablation$_{\!}$ studies$_{\!}$} on$_{\!}$ UnAV-100$_{\!}$~\cite{geng2023dense}$_{\!}$ (see$_{\!}$ \S\ref{sec44}). The$_{\!}$ adopted$_{\!}$ network$_{\!}$ designs$_{\!}$ are$_{\!}$ marked$_{\!}$ in$_{\!}$ bold.}
\end{table*}

==> tabs/algorithm_LCC.tex <==
% \captionsetup[algorithm*]{skip=3pt}
\begin{algorithm}[h]
    % \captionsetup[algorithm]{aboveskip=0.2cm, belowskip=-0.3cm}
    \caption{Pseudo-code of Locality-aware Correspondence Correction (LCC) in a PyTorch-like style.}
   
    \label{alg:code}

    \definecolor{codeblue}{rgb}{0.25,0.5,0.5}
    \lstset{
     backgroundcolor=\color{white},
     basicstyle=\fontsize{9pt}{9pt}\ttfamily\selectfont,
     columns=fullflexible,
     breaklines=true,
     captionpos=b,
     escapeinside={(:}{:)},
     commentstyle=\fontsize{9pt}{9pt}\color{codeblue},
     keywordstyle=\fontsize{9pt}{9pt},
     numbers=none % Disable line numbering
     %  frame=tb,
    }
   \begin{lstlisting}[language=python]
# F_v: visual features from multimodal input encoding modules(B, T, D) 
# F_a: audio features from multimodal input encoding modules(B, T, D)  
# B: batch size
# T: number of segments
# D: embedding dimension
# tau: a learnable temporal parameter
# sigma: a learnable standard deviation 
# pi: the ratio of a circle's circumference to its diameter

(:\color{codedefine}{\textbf{def}}:) (:\color{codefunc}{\textbf{Calculate\_LCC}}:) (F_v, F_a, tau, sigma):
    # calculate similarity matrix
    F_v = F_v.(:\color{codepro}{\textbf{reshape}}:)(B x T, D) # (B x T, D)
    F_a = F_a.(:\color{codepro}{\textbf{reshape}}:)(B x T, D) # (B x T, D)
    sim_v2a = F_v @ F_a.(:\color{codepro}{\textbf{transpose}}:)(0, 1) / tau
    sim_a2v = F_a @ F_v.(:\color{codepro}{\textbf{transpose}}:)(0, 1) / tau
       
    # calculate correspondence objective G (B x T, B x T)
    G = (:\color{codeorg}{\textbf{zeros}}:)((B x T, B x T)) # (B x T, B x T)
    (:\color{codedefine}{\textbf{for}}:) i (:\color{codedefine}{\textbf{in}}:) (:\color{codedefine}{range}:)(0, B x T, T):
        G_T = (:\color{codefunc}{\textbf{Gaussian}}:)(T, sigma)
        G[i : i + T, i : i + T] = G_T
           
    # to align visual modality with audio modality
    LCC_v2a = -(:\color{codeorg}{\textbf{sum}}:)((:\color{codeorg}{\textbf{log\_softmax}}:)(sim_v2a, dim=1) * G, dim = 1).(:\color{codeorg}{\textbf{mean}}:)()
    # to align audio modality with visual modality
    LCC_a2v = -(:\color{codeorg}{\textbf{sum}}:)((:\color{codeorg}{\textbf{log\_softmax}}:)(sim_a2v, dim=1) * G, dim = 1).(:\color{codeorg}{\textbf{mean}}:)()
       
    # calculate final LCC
    LCC = (LCC_v2a + LCC_a2v) / 2
    return LCC

# calculate correspondence objective within the same video (T, T)
(:\color{codedefine}{\textbf{def}}:) (:\color{codefunc}{\textbf{Gaussian}}:) (T, sigma):
    G_T = ((:\color{codedefine}{arange}:)(T).(:\color{codepro}{\textbf{reshape}}:)(T, 1) - (:\color{codedefine}{arange}:)(T).(:\color{codepro}{\textbf{reshape}}:)(1, T)) / (:\color{codeorg}{\textbf{sqrt}}:)(2) # (T, T)
    G_T = - (G_T**2) / 2.0 / (sigma**2)
    G_T = 1 / (sigma * (:\color{codeorg}{\textbf{sqrt}}:)(2 * pi)) * (:\color{codeorg}{\textbf{exp}}:)(G_T)
       return G_T
   \end{lstlisting}
    % \end{minipage}
   % \end{algorithm}
\end{algorithm}

